A CMOS-compatible Ising Machine with Bistable Nodes

Physical Ising machines rely on nature to guide a dynamical system towards an optimal state which can be read out as a heuristical solution to a combinatorial optimization problem. Such designs that use nature as a computing mechanism can lead to higher performance and/or lower operation costs and hence have attracted research and prototyping efforts from industry and academia. Quantum annealers are a prominent example of such efforts. However, some physics-centric Ising machines require stringent operating conditions that result in significant bulk and energy budget. Such disadvantages may be acceptable if these designs provide some significant intrinsic advantages at a much larger scale in the future, which remains to be seen. But for now, integrated electronic designs of Ising machines allow more immediate applications. We propose one such design that uses bistable nodes, coupled with programmable and variable strengths. The design is fully CMOS compatible for chip-scale applications and demonstrates competitive solution quality and significantly superior execution time and energy.

==> Sections/7bio.tex <==
\vspace{-1.5cm}
\begin{IEEEbiography}
    [{\includegraphics[width=1.0in,height=1.5in,clip,keepaspectratio]{rka.JPG}}]{Richard Afoakwa}
    received the BS degree in electrical engineering from the University of Maryland, College Park, MD, in 2011. He is pursing the PhD in electrical engineering from the University of Rochester, Rochester, NY. His research interests include high performance and energy efficient computer architecture.
\end{IEEEbiography}
\vspace{-1.5cm}
\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{wesley.jpeg}}]{Yiqiao Zhang}
    received the BS degree in electrical engineering from the University of Illinois at Urbana-Champaign, Champaign, IL, in 2015, and the MS degree in electrical engineering from the University of Rochester, Rochester, NY, in 2016. He is working toward the PhD degree in electrical engineering from the University of Rochester. His research interests include wideband and high-resolution A/D converters.
\end{IEEEbiography}
\vspace{-1.5cm}
\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Anshujit.jpeg}}]{Anshujit Sharma}
    received the B. Tech. degree in electronics and communication engineering from National Institute of Technology Silchar, India, in 2016. He is pursuing PhD in electrical engineering from the University of Rochester, NY. His research interests include high performance computer architectures and nature based computing.
\end{IEEEbiography}
\vspace{-1.5cm}
\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,clip]{zi.jpeg}}]{Zeljko Ignjatovic}
    received the BS degree in electrical engineering from University of Novi Sad, Serbia, and the MS and PhD degrees in electrical engineering from University of Rochester, NY, in 1999, 2001, and 2004, respectively. He is currently an Associate Professor of Electrical and Computer Engineering at University of Rochester. His areas of interest include analog circuit design and development of A/D converters, image sensor architectures, radar and ultrasound imaging techniques and related signal processing methods.
\end{IEEEbiography}
\vspace{-1.0cm}
\begin{IEEEbiography}
    [{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mch.jpg}}]{Michael Huang}
    received the BS degree in computer science and engineering from Tsinghua University, Beijing, in 1994, the MS and the PhD degree in computer science from University of Illinois at Urbana-Champaign in 1999 and 2002, respectively. From 1994 to 1997, he was a lead architect in building a 32-processor hierarchical shared-memory multiprocessor research prototype. He joined the faculty of the Electrical and Computer Engineering department in 2002. In 2010, he was on sabbatical at IBM T. J. Watson Research Center working on future POWER processor concept development. His research interests include various aspects of high-performance computer architecture such as processor microarchitecture, communication and memory substrate, reliability, and energy-efficient and complexity-effective design. His is particularly interested in addressing emerging issues and exploring new capabilities in the underlying device, circuit, and manufacturing technology. He is a recipient of the NSF CAREER award and a member of the IEEE and the ACM.
\end{IEEEbiography}

